Adversarial purification with Score-based generative models

While adversarial training is considered as a standard defense method against adversarial attacks for image classifiers, adversarial purification, which purifies attacked images into clean images with a standalone purification model, has shown promises as an alternative defense method. Recently, an Energy-Based Model (EBM) trained with Markov-Chain Monte-Carlo (MCMC) has been highlighted as a purification model, where an attacked image is purified by running a long Markov-chain using the gradients of the EBM. Yet, the practicality of the adversarial purification using an EBM remains questionable because the number of MCMC steps required for such purification is too large. In this paper, we propose a novel adversarial purification method based on an EBM trained with Denoising Score-Matching (DSM). We show that an EBM trained with DSM can quickly purify attacked images within a few steps. We further introduce a simple yet effective randomized purification scheme that injects random noises into images before purification. This process screens the adversarial perturbations imposed on images by the random noises and brings the images to the regime where the EBM can denoise well. We show that our purification method is robust against various attacks and demonstrate its state-of-the-art performances.

==> backups/ChE_MoreDatasets.tex <==
\section{Full list of defense results for extra datasets}
\label{sec:extensive}
\input{tables/extensive}
We present the full list of defense results for various datasets, including MNIST, FashionMNIST, and CIFAR-100 in~\cref{table:extensive}.
As we mentioned in~\cref{sec:extra}, 

==> backups/methods_old.tex <==
\section{Adversarial purification with score-based generative models}
\label{sec:methods}

\begin{figure*}[!htb]
  \centering
  \includegraphics[width=0.8\textwidth]{./figures/network.png}
  \caption{Overview of our algorithm.}
  \label{fig:network}
\end{figure*}

\subsection{Training score network with \gls{dsm}}


\label{sec:learningscore}
Recently, generating samples from a target distribution trained with denoising score matching~\citep{Song2019NCSN, ho2020ddpm, joli2021asm} has achieved high performance, and convergence to the target distribution is guaranteed. 
In this section, we introduce our purification model trained with \emph{score-based generative models}.
% 여기서는 NCSN을 train한다. NCSN은 annealed Langevin sampling라고 불리는 variant of SGLD를 이용한 sampling method를 통해서 model distribution에서 data를 sampling하는 방법이다. 이것이 작동하게 하기 위해선,ㄴ 여러 noise level에서 동시에 작동하는 score network의 설계가 핗요하다. Original version에서 각각의 noise level에 대해서 별개의 score network를 설계했지만, 저자들은 joint 
%Annealed Langevin sampling을 수행하기 위해서는, 서로 다른 noise level에서의 model distribution의 overlap이 커서 연계될 수 있 
For training the purification models, we use the recently proposed \gls{ncsn} \cite{Song2019NCSN}, a score-based generative model that takes advantage of various noise level of \glspl{dsm}. We choose \gls{ncsn}v2 \cite{Song2020NCSNv2}, the updated version of \gls{ncsn} that improves the image generation quality and stabilizes the optimization process to the original work. The updated \gls{ncsn}v2 refines the score network to a single model $s_\theta:\mathbb{R}^D\to\mathbb{R}^D$ by incorporating all Gaussian noise levels and minimize the weighted sum of denoising score matching objective \eqref{eq:dsm_denoising}.
The original paper took the weight of each noise level $\lambda(\sigma)=\sigma^2$, by equalizing losses of all noise level $\sigma_i$'s at the training phase. Then the marginal objective with respect to all noise level is
\begin{equation}
\mathcal{L}(\theta, \{\sigma_i\}_{i=1}^L )=\sum_{i=1}^L \sigma_i ^2 l(\theta, \sigma_i)
\end{equation}
where $\{\sigma_i\}_{i=1}^L$ are the chosen noise levels. The largest noise level $\sigma_1$ is set to the maximum $l_2$ distance between two data points in the training dataset for better mixing, and the smallest noise level $\sigma_L$ is set sufficiently small to converge 

 * Adversarially training NCSN part

For purifying the adversarial example with respect to a particular threat model, we augment the adversarial examples to the training dataset. Let $A(x)$ be an attacked example, whose natural counterpart is set to $x$. Then the goal is to specialize the adversarial attack $A$ into the data manifold, by training the approximate score function of attacked examples. The adversarial loss function that substitutes \eqref{eq:4} is given by   
\begin{align}\label{eq:4}
l_\text{adv}(\theta, \sigma)
= \frac{1}{2} \mathbb{E}_{p_\text{data}(x)} \mathbb{E}_{\mathcal{N}(x'|A(x),\sigma^2 I)}\left[\left\lVert s_{\theta} (x')+\frac{x-x'}{\sigma}\right\rVert_2^2\right]
\end{align}

%\textcolor{red}{(While $A(x)$ should be a set of possible attacks in the threat model, I described it as a single-output function because of lack of space.)}
Minimizing the loss $\sum_{i=1}^L \sigma_i ^2 l_{adv}(\theta, \sigma_i )$ will learn the score function which consist of natural examples with high density and adversarial ones with low density. %low energy and adversarial examples with high energy.
% At the training phase, the largest noise level is 50 and the smallest noise level is 0.0085 for training generative model for CIFAR-10.
%\subsection{Noise injection before purification, with deterministic short-term dynamics}


\subsection{Purification via iterative score matching}
We introduce our deterministic sampling strategy that purifies the adversarial attack. Given the purifier $s_{\theta}$ and the classifier $g_\phi$ networks, we iteratively propagate the input into the purifier network to refine attacked images. We denote the weight of $i$-th refinement step to $\alpha_i$. The purifier $s_{\theta}$ is learned by score matching methods mentioned above. The step size $\alpha_i$ can be either pre-trained when the targeted threat model is restricted, or can be obtained by adaptation. The overall algorithm is outlined at Algorithm \ref{alg:example}. 

Then the score network is learned by minimizing \eqref{eq:4}, the score function $s_{\theta}(x)$ approximates the log density function $\nabla_x \log p_{\theta} (x)$. So adding instantaneous vector in the direction of $s_{\theta} (x)$ increases the data density. The step size $\alpha_i$ for $i$-the iteration is either pre-trained from validation set or obtained from adaptive strategy. In order to avoid outliers and get consistent prediction result, we get the ensemble average of pre-softmax layer as $\hat{y} = {\arg\max}_{j\in[K]} (\sum_{i=1}^K {z_i})_{j}$. The overall algorithm is outlined at Algorithm \ref{alg:example}.
\begin{algorithm}[tb]
   \caption{Purification strategy}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $x_0$, score network $s_\theta$, classifier $f_\phi$, injecting noise scale $\sigma$, number of different noises $N$, step size $\{\alpha_i\}_{i=1}^L$ if pre-trained, step size rate $\alpha$ if not
   \FOR{$j=1$ {\bfseries to} $N$}
   \STATE {$x_{0,i} \gets \prod_{[0,1]^D}(x_0 + \sigma n_i)$, $n_i\sim\mathcal{N}(0,I)$}
   \FOR{$j=1$ {\bfseries to} $L$}
   \IF {$\alpha_j$ not pre-trained}
      \STATE $x_{j,i} ' \gets x_{j,i} + \epsilon s_{\theta} (x_{j,i})$
      \STATE $\alpha_j \gets \frac{\alpha\epsilon}{1-\frac{s_\theta (x_{j,i}) \cdot s_\theta (x_{j,i} ')}{\norm{s_\theta (x_{j,i})}_2^2}}$
      \STATE 
   \ENDIF
   \STATE {$x_{j,i} \gets x_{j-1,i} + \alpha_{j} s_{\theta} (x_{j,i})$}
   \STATE {$z_{j,i} = g_{\phi} (x_{j,i})$}
   \ENDFOR
   \ENDFOR
   \STATE $\hat{y} = {\arg\max}_{k\in[K]} (\sum_{j=1}^L {z_j})_{k}$
   \STATE {\bfseries Return} Output label $\hat{y}$, Purified data $x_L$
\end{algorithmic}
\end{algorithm}

\subsection{Auxiliary module: setting adaptive or deterministic step size}\label{sec:lr}
In the purification stage, the step size at each iteration $\alpha_i$ is pre-trained from validation set, assuming that the threat model is given. However, in many realistic situation, we should take account of adaptive step sizes. We assume that the distribution learned by the score network is mixture of Gaussian distribution, whose centroids are located at each data point. Let such data point be $x$, for example. We assume that the distribution near $x$ is given by $\mathcal{N}(x,\sigma_x^2 I)$ since every data lies on a very high-dimensional vector space.

Then, for calculating $\sigma_x$, we move $x$ for a little amount of the direction of score function $s_{\theta} (x)$, as $x'=x+\epsilon s_{\theta} (x)$. Then we project the score function at $x'$ to the direction of $x_{\theta} (x)$, to detect how much amount of $s_{\theta}(x)$ shrinks by instantaneous change of data point. We project $s_{\theta} (x')$ to $s_{\theta} (x)$ as $s_{\theta}^{\Pi} (x') = s_{\theta} (x) \frac{s_{\theta}(x')\cdot s_{\theta}(x)}{\norm{s_{\theta}(x)}_2^2}$. Then we measure how much amount of $s_{\theta}(x)$ component is applied to derive $\alpha_i$.

Let $\alpha$ be the \textit{step size rate}, one-step relative speed of convergence. For example, when $\alpha=1$, then $x$ moves to the local minimum of $s_{\theta}$ at once, assuming that the data distribution is unimodal Gaussian. When $\alpha_i$ is the step size at $i$-th iteration, then the following holds.
\begin{equation}
\frac{\alpha_i}{\epsilon}=\frac{s_{\theta}(x)\left(1-\frac{s_{\theta}(x)\cdot s_{\theta}(x')}{\norm{s_{\theta}(x)}_2^2}\right)}{\alpha s_{\theta} (x)}
\end{equation}
As a result, the adaptive step size is obtained by $\alpha_i = \frac{\alpha\epsilon}{1-\frac{s_\theta (x_i) \cdot s_\theta (x_i ')}{\norm{s_\theta (x_i)}_2^2}}$. 






==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> tables/correctbpda.tex <==
\begin{table}[!htb]
\centering
\caption{Corrected robust accuracy on \gls{bpda} attack on CIFAR-10 dataset.}\label{table:correctbpda}
\begin{tabular}{lllllll}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Accuracy (\%)}  \\
 & Natural & Robust  \\
 \midrule
 $\sigma=0.1$ & 92.64 & {\color{red} 48.28} \\
 $\sigma=0.15$ & 89.19 & 62.00 \\
 $\sigma=0.2$ & 85.47 & 69.67 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/morepb.tex <==
\begin{table}[!htb]
\caption{\label{table:pbfull}Evaluation results for preprocessor-blind attacks without noise injection and deterministic step sizes, starting with $\alpha_1=0.08$ and $\alpha_L=8.0\times 10^{-4}$ with $L=10$. Threat model: $l_\infty$ $\epsilon$-ball with $\epsilon=8/255$, CIFAR-10 dataset.}
\centering
\begin{tabular}{lllllll}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Accuracy (\%)} & \multicolumn{2}{c}{Network architecture} & \multicolumn{2}{c}{Attack configuration} \\
\cmidrule{2-3}\cmidrule{4-5}\cmidrule{6-7}
 & Natural & Robust & Purifier & Classifier & Attack method & Threat blindness\\
 \midrule
ADP & & & & & \\
\hspace{3mm}Naturally Trained & 91.89 & 81.84 & \gls{ncsn}v2 & WRN-28-10 & Classifier \gls{pgd} & Unseen\\
\hspace{3mm}Naturally Trained & 91.90 & 82.96 & \gls{ncsn}v2 & WRN-28-10 & Classifier BIM & Unseen\\
\hspace{3mm}AT ($\epsilon=4/255$) & 91.90 & 90.59 & \gls{ncsn}v2 & WRN-28-10 & Classifier \gls{pgd} &Seen \\
\hspace{3mm}AT ($\epsilon=4/255$) & 91.90 & 88.46 & \gls{ncsn}v2 & WRN-28-10 & Classifier BIM & Seen\\
\hspace{3mm}AT ($\epsilon=8/255$) & 91.39 & {92.36} & \gls{ncsn}v2 & WRN-28-10 & Classifier \gls{pgd} &Seen\\
\hspace{3mm}AT ($\epsilon=8/255$) & 91.39 & 92.18 & \gls{ncsn}v2 & WRN-28-10 & Classifier BIM & Seen\\
\hspace{3mm}AT ($\epsilon=16/255$) & 91.73 & 89.58 & \gls{ncsn}v2 & WRN-28-10 & Classifier \gls{pgd} & Seen\\
\hspace{3mm}AT ($\epsilon=16/255$) & 91.73 & 89.81 & \gls{ncsn}v2 & WRN-28-10 & Classifier BIM & Seen\\
\hspace{3mm}Natural ($\sigma=0.15$) & 89.60 & 82.98 & \gls{ncsn}v2 & WRN-28-10 & Classifier \gls{pgd} & Unseen \\
\midrule
\citep{hill2020stochastic} & 84.12 & 78.91 & IGEBM & WRN-28-10 & Classifier \gls{pgd}&Unseen\\
\citep{shi2021online} & 84.07 & 51.42 & Self-supervised & ResNet-18 & Classifier \gls{pgd} & Unseen \\
\citep{shi2021online} & 91.89 & 53.58 & Self-supervised & WRN-28-10 & Classifier \gls{pgd} & Unseen \\
\citep{song2018pixeldefend} & 90 & 70 & PixelCNN & ResNet-62 & Classifier \gls{pgd} & Seen \\
\bottomrule
\end{tabular}
\end{table}

==> tables/noensemble.tex <==
\begin{table}
\caption{Evaluation results for various attacks without ensemble over purification runs.}\label{table:noensemble}
\centering
\begin{tabular}{llllll}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Accuracy (\%)} &  \multirow{2}{*}{Architecture} \\
 & Natural & Robust &  & \\
 \midrule
ADP & 91.89 & & \\
\hspace{3mm}Classifier PGD & & 81.84 &  WRN-28-10 \\
\hspace{3mm} BPDA & & {\color{red} 48.24} & WRN-28-10 \\
\hspace{3mm}Unrolling & & 78.49 & WRN-28-10 \\
\hspace{3mm}Approx. Input & & 72.73 &  WRN-28-10 \\
\hspace{3mm}Joint (one) & & 78.98 & WRN-28-10 \\
\hspace{3mm} Joint (full) & & 77.24 &   WRN-28-10 \\
\hspace{3mm} SPSA & & 79.64 &  WRN-28-10 \\
\bottomrule
\end{tabular}
\end{table}

==> xr.tex <==

\usepackage{xr}
\makeatletter
\newcommand*{\addFileDependency}[1]{%
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[2]{%
    \externaldocument[#1]{#2}%
    \addFileDependency{#2.tex}%
    \addFileDependency{#2.aux}%
}
